Towards Distributed Energy Services: Decentralizing Optimal Power Flow with Machine Learning

The implementation of optimal power flow (OPF) methods to perform voltage and power flow regulation in electric networks is generally believed to require extensive communication. We consider distribution systems with multiple controllable Distributed Energy Resources (DERs) and present a data-driven approach to learn control policies for each DER to reconstruct and mimic the solution to a centralized OPF problem from solely locally available information. Collectively, all local controllers closely match the centralized OPF solution, providing near optimal performance and satisfaction of system constraints. A rate distortion framework enables the analysis of how well the resulting fully decentralized control policies are able to reconstruct the OPF solution. The methodology provides a natural extension to decide what nodes a DER should communicate with to improve the reconstruction of its individual policy. The method is applied on both single- and three-phase test feeder networks using data from real loads and distributed generators, focusing on DERs that do not exhibit inter-temporal dependencies. It provides a framework for Distribution System Operators to efficiently plan and operate the contributions of DERs to achieve Distributed Energy Services in distribution networks.

==> controlperspective.tex <==
\section{A Control-Theoretic Lens for OPF}

The dynamics considered in OPF for electric distribution systems with alternating current (AC) are typically not described with differential equations, as these are assumed to be in a \emph{quasi steady-state}. 
This assumption rests on the condition that the distribution network is connected to the transmission grid through a substation, which can be modeled as an \emph{infinite} bus, meaning that the transmission grid \emph{admits} or \emph{compensates} any changes in power across the distribution network to enable a \emph{fixed} voltage phasor.
With this assumption, voltage and power flow across a network can be determined through solving a set of algebraic equations describing fundamental first principles in electric power.

However, when we consider decentralized control solutions, the spatial coupling and the updating nature of local controllers requires a dynamical analysis.
We adopt and extend a control-theoretic perspective to optimal power flow (OPF), as initially proposed in~\cite{wang_control_2011} for general optimization algorithms and interpreted for power systems in~\cite{hauswirth_online_2017}.
This lens will help us interpret the challenge of decentralizing OPF with machine learning and it naturally triggers relevant questions around the analysis, development and integration of our solution.

In control theory, the state-space representation a \emph{dynamical system} can be thought of as described by a set of variables including input, state and output variables~\cite{friedland_control_2012}, related by a set of differential and/or algebraic equations. 
The input variables are also called \emph{exogenous} as these typically enter from outside the system boundary, and can be split up in \emph{controllable} input variables~$u\in \mathcal U$ (in short, ``inputs'') and \emph{uncontrollable} input variables~$d \in \mathcal D$ (in short, ``disturbances'').
The state variables~$x \in \mathcal X$ (or ``states'') are all the variables necessary to mathematically describe the system's full dynamics.
The states may contain certain inputs or disturbances. 
The remaining states, those that are not inputs or disturbances, but that are needed to describe the system dynamics are \emph{endogenous} variables.
Endogenous variables have values that are determined by other exogenous variables in the system, and are often called \emph{dependent} variables, such as in econometrics~\cite{greene_econometric_2000}.
The output variables~$z \in \mathcal Z$ (or ``outputs'') are all the variables that are measured in some \emph{real-time} capacity, potentially at various sampling-rates.

Consider a network modeled by a graph~$\G = (\N,\E)$ with $\N$ a set of nodes representing all buses with cardinality~$\nu := |\N|$ and $\E$ a set of edges representing all branches with cardinality~$\eta := |\E|$.
At each bus, we have 4 variables; voltage magnitude~$V_n$, voltage angle~$\delta_n$, and nodal real and reactive power~$p_n$~and~$q_n$, for all $n \in \N$. Vectorized for all buses, we have~$V,\delta,p,q \in \R^{\nu}$ and we define the state of the system as
\begin{equation}
x := 
\left[
\begin{matrix}
V \\
\delta \\
p \\
q \\
\end{matrix} 
\right] 
\in \R^{4 \nu} \,.
\label{eqn:state}
\end{equation}

As suggested above, we partition the state~$x$ into controllable inputs~$u$, uncontrollable inputs or disturbances~$d$ and endogenous variables~$x^{\text{end}}$.
This partitioning is done per bus, based on the bus type, as suggested in~\cite{hauswirth_online_2017} and summarized in Table~\ref{tab:bus_types}. 

\begin{table}[h]
\centering
\begin{tabular}{lccc} 
\toprule
 				& \multicolumn{2}{c}{Exogenous} 			& Endogenous 		\\ \cmidrule(r){2-3}
				& Controllable - $u$	& Uncontrollable - $d$ 	& 	$x^{\text{end}} := x_{\backslash \{ u,d \} }$			\\ \midrule
PQ generation		& $p_n,q_n$		&					& $V_n,\delta_n$	\\
PQ load			& 				& $p_n,q_n$			& $V_n,\delta_n$	\\
PV generation		& $p_n,V_n$		& 					& $q_n, \delta_n$	\\
slack bus			& $V_0$			& $\delta_0$			& $p_0,q_0$		\\ \bottomrule
\end{tabular}
\caption{Partitioning of nodal variables for all bus types.}
\label{tab:bus_types}
\end{table}

Note that the exogenous inputs are also treated as state variables: ~$\{u,d\} \subset x$. 
In our setting, the state $x$ is the solution to either a set of algebraic equations or an optimization problem. In the former case, we have to solve the power flow equations $F(x) = 0$ to find $x$,
\begin{equation}
x \in \{ \xi \in \R^{4\nu} \ : \ F(\xi) = 0  \} =: \mathcal M \,.
\end{equation} 
Here, $\mathcal M$ is the \emph{power flow manifold}, as properly defined in~\cite{bolognani_fast_2015}, representing all equations in Section~\ref{sec:opf} needed to represent power flow physics and operating constraints.

\usetikzlibrary{shapes,arrows}
\tikzstyle{block} = [draw, fill=white, rectangle, 
    minimum height=3em, minimum width=6em]
\tikzstyle{sum} = [draw, fill=white, circle, node distance=1cm]
\tikzstyle{input} = [coordinate]
\tikzstyle{connect} = [coordinate]
\tikzstyle{output} = [coordinate]
\tikzstyle{state} = [coordinate]
\tikzstyle{disturbance} = [coordinate]
\tikzstyle{pinstyle} = [pin edge={to-,thin,black}]

\begin{figure*}[h!]
\centering
\begin{tikzpicture}[auto, node distance=2cm,>=latex']

	\node [connect, name=input_ff] (reference_z) {};
	\node [connect, right of=reference_z, node distance=1cm] (connect1) {};
 	\node [connect, below of=connect1, node distance=2.5cm] (connect5) {};
	\node [block, right of=connect1, align=center, node distance=2cm] (feedforward) {Feedforward \\ Controller};
    	\node [sum, right of=feedforward, node distance=3cm] (sum1) {};
	\node [input, above of=sum1, node distance=1cm] (input_ol) {};
	\node [block, right of=sum1, node distance=3cm] (system) {System};
     	\node [input, above of=system, node distance=1cm] (connect2) {};
	\node [input, above of=connect2, node distance=0.5cm] (disturbance) {};
    	\node [block, below of=system, node distance=1.5cm, align=center] (feedback_x) {Feedback \\ Controller};
% 	\node [block, below of=system, node distance=4.25cm, align=center] (feedback_z) {Output \\ Feedback \\ Controller};
% 	\node [connect, left of=feedback_z, node distance=4.5cm] (connect3) {};
% 	\node [connect, above of=connect3, node distance=3cm] (connect4) {};
    	\node [sum, right of=feedback_x, node distance=2cm] (sum2) {};
%	\node [input, below of=sum2, node distance=3.5cm] (reference_x) {};
	\node [block, right of=system, node distance=5cm] (sensors) {Sensors};
     	\node [block, right of=feedback_x, node distance=5cm, align=center] (estimator) {State \\ Estimator};
	\node [output, right of=sensors, node distance=2cm] (output) {};
% 	\node [sum, below of=output, node distance=4.25cm] (sum3) {};
 	\node [connect, below of=sum2, node distance=1cm] (connect6) {};
	\node [output, right of=output, node distance=1cm] (exit) {};
	 
	 \draw [->] (disturbance) -- node[pos=0.1] {$d$} (system);
%	 \draw [->] (connect2) -| (connect1) |- (feedforward);
	 \draw [->] (connect2) -| (feedforward);
	 \draw [->] (feedforward) -- node{$u^{\text{ff}}$} (sum1);
% 	 \draw [->] (input_ol) -- node{$u^{\text{ol}}$} (sum1);
    	\draw [->] (sum1) -- node {$u$} (system);
    	\draw [->] (system) -- node [name=x] {$x^{\text{end}}$}(sensors);
    	\draw [->] (sensors) -- node [name=z] {$z$} (exit);
    % 	-- node[pos=0.99] {$-$} (sum3);
        \draw [->] (output) |- (estimator);
        \draw [->] (reference_z) -- node {$r_x$} (feedforward);
        \draw [->] (estimator) -- (sum2);
        \draw [->] (estimator) --  node {$\hat{x}^{\text{end}}$} node[pos=0.9] {$-$} (sum2);
%        \draw [->] (reference_x) -- node[pos=0.9]{$r_x$} (sum2);
        \draw [->] (sum2) -- (feedback_x);
        \draw [->] (feedback_x) -| node[pos=0.7] {$u^{\text{fb}}$} (sum1);
%        \draw [->] (sum3) -- (feedback_z);
%        \draw [->] (feedback_z) -- (connect3) -- node[pos=0.5] {$u^{\text{fb}}_z$} (connect4) -- (sum1);
       \draw [->] (connect1) -| (connect5) -- (connect6) -- node[pos=0.65]{$r_x$} (sum2);
%        \draw [->] (output) -- (exit);
        
\end{tikzpicture}
\caption{Dynamical system representation with feedback and feedforward control.} \label{fig:combined_fb_ff}
\end{figure*} 
 
% \todo[inline]{Consider only explaining feedforward here.}
Figure~\ref{fig:combined_fb_ff} shows a block diagram of a general dynamical system, depicting with both feedback and feedforward control. 
In feedback control, the output~$z$ is used in real-time to inform the input~$u$ of the system, typically by comparing~$z$ to some defined reference signal or set point~$r$. An example is the use of voltage measurements across a distribution network to automatically adjust the feeder voltage through controlling the load tap changer. 
In this context, the state vector~$x$ may not be fully measured in the output~$z$, and an \emph{state estimator} or \emph{observer} is needed to estimate the full state~$\hat{x}$ from the output. 
Feedforward control is traditionally known as a simple and powerful technique to complement feedback control. It can be used both to improve the response to reference signals and to reduce the effect of measurable disturbances~\cite{astrom_feedback_2010}. 
As such, there are broadly two forms of feedforward control. Firstly, a reference (either on output~$r_z$ or state~$r_x$) can be used to determine an input~$u_r^{\text{ff}}$ that \emph{anticipates} the system's dynamical response, typically by feeding~$r_z$ through an \emph{inverse model} of the system. Secondly, information about the disturbances~$d$, either through real-time measurement or a prediction, may be used to design an input~$u_d^{\text{ff}}$ that tries to compensate for its harmful effects by \emph{attenuating} it directly or, again, \emph{anticipating} the system's dynamical response.

By combining feedforward and feedback control in the right way, one has two degrees of freedoms to split the control design problem into two parts. The feedback controller can be designed to give robustness and effective disturbance attenuation, and the feedforward part can be designed independently to give the desired response to command signals or objectives~\cite{astrom_feedback_2010}.

In this paper, we direct our focus on using machine learning to design a \emph{decentralized feedforward controller}~$\hat u_i := \hat \pi_i (d_i) \ \forall i \in \C$ that locally reconstructs the optimal actions of an OPF problem~$u^*_i$ from measurable disturbances~$d_i$, as given in Table~\ref{tab:bus_types} for different bus types. For a general dynamical system, the method can be interpreted as \emph{learning-based feedforward optimization}~\cite{dobbe_fully_2017,dobbe_feedforward_2018}. 
For this paper, we do not consider using machine learning to learn a feedback controller; a policy $\hat u_i := \hat \pi_i (x_i^{\text{end}})$ that is a function of endogenous dynamic state variables, as proposed in~\cite{bellizio_optimized_2017}. 
The main challenge with using these variables is that the historical data of $x_i^{\text{end}}$ will be different than the measured state $x_i^{\text{end}} = f(u_i,d_i)$, which is a function of the input. 
This requires understanding existence and stability of the fixed point solution~$(x^{+,\text{end}}_i,\hat u^+_i)$ such that $x_i^{+,\text{end}} = f(u^+_i,d_i)$ and $\hat u^+_i = \hat \pi_i(x_i^{+,\text{end}})$. 
If the historical data was affected by control actions, careful analysis is necessary to deal with potential issues related to closed-loop identification~\cite{van_den_hof_closed-loop_1998}. 


==> interpretMLmodels.tex <==
\section{Interpreting the Machine Learning Models}
\label{subsec:interpretation}
In this section, we analyze how the structure of different learned controllers~$i,j \in \C$ differ across the network as reflected by parameters~$\beta^{(i)},\beta^{(j)}$ in (17) of the main manuscript. What does this tell us about the network and OPF problem?

In our first case study, we determined regression models for 27 different inverters. Table \ref{tab:InvMdl} shows regression results for inverters A and B (both indicated in Figure 3 of the main manuscript). The first two columns present the  features selected by the stepwise regression and the values for the $\beta$-coefficients in (17) of the main manuscript. The third column shows the standard error of the estimate, and the fourth lists p-values, which here means the probability that coefficient is zero. A p-value of 0.1 implies a 10\% chance that the corresponding coefficient is zero. Note how the stepwise regression approach results in two clearly different models.
The reactive power output of inverter A depends predominantly on the local reactive power consumption $\varphi^{(A)}_2$, while the output of inverter B is strongly related to the reactive power capacity $\varphi^{(B)}_3$ and $\varphi^{(B)}_2$ is less relevant.
Inverter A's structure can be explained by the fact it is located at the end of the feeder. As a result, the aggregate power flow at A is relatively low and correlated with A's own consumption. As the objective is to minimize losses and voltage deviations, A tries to produce a signal that looks like providing the neighboring demand for reactive power, thereby minimizing current locally \emph{and} upstream.
Inverter B's structure can be explained by its location close to the feeder head. In this area, the aggregate power flow is much larger, and the output of inverter B is needed more as a ``bulk'' product to lower the flow on branches elsewhere in the network.
This causes inverter B to operate at its maximum capacity most of the time, causing correlation with the output.
As the maximum capacity varies with the local real power generation at B (a constraint formulated in~(11) of the main manuscript), the learning algorithm tries to ``listen closely'' to the present maximum capacity.
This example illustrates that optimal reactive power output of two inverters can have a completely different structure. Therefore, effective design of controllers based on local measurements is challenging, and can benefit from a data driven approach. 
%\begin{figure}[!t]
%\centering
%\includegraphics[width=.5\textwidth]{rbic_figs/RegResultInv3.png}
%\caption{Table with normalized regression model for Inverter A. The columns refer to the $\beta$ coefficients of \eqref{eq:MLRmodel}, with SE the standard error, and pValue is the probability that the coefficient is zero.}
%\label{tab:RegResultInv3}
%\end{figure}
%
%\begin{figure}[!t]
%\centering
%\includegraphics[width=.5\textwidth]{rbic_figs/RegResultInv14.png}
%\caption{Table with normalized regression model for Inverter number B. \todo[inline]{Make real tables} }
%\label{tab:RegResultInv14}
%\end{figure}
\begin{table}[!t]
\renewcommand{\arraystretch}{1.3}
\caption{Normalized regression coefficients for inverter A and B, as depicted in Figure~\ref{fig:FeederDiag}.}
\label{tab:InvMdl}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c c c c || c c c c}
\hline
A & Est. & SE & p-value &  B & Est. & SE & p-value \\
\hline\hline
offset	&	0.02	&	0.01	&	0.01				&	offset	&	0.02	&	0.00	&	$8.2 e^{-4}$ \\
$\varphi_1$	&	0.37	&	0.01	&	$0$		&	$\varphi_1$	&	0.04	&	0.00	&	$3.2e^{-22}$ \\
$\varphi_2$	&	0.77	&	0.01	&	0				&	$\varphi_3$	&	0.96	&	0.01	&	0 \\
$\varphi_3$	&	-0.21	&	0.02	&	$8.0e^{-24}$		&	$\varphi_1 \varphi_3$	&	0.06	&	0.01	&	$1.2e^{-12} $\\
$\varphi_1 \varphi_2$	&	0.17	&	0.01	&	$0$		&	$\varphi_1^2$	&	-0.03	&	0.00	&	$3.9e^{-14}$\\
$\varphi_1^2$	&	-0.06	&	0.01	&	$1.4e^{-12}$		&	$\varphi_3^2$	&	-0.03	&	0.01	&	$6.1e^{-9}$ \\
\hline
\end{tabular}%
}
\end{table}

% \begin{table}[!t]
% \renewcommand{\arraystretch}{1.3}
% \caption{Normalized regression coefficients for inverter A and B, as depicted in Figure~\ref{fig:FeederDiag}.}
% \label{tab:InvMdl}
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{c c c c c c c c c c c}
% \hline
%  & 1 & $\varphi_1$ & $\varphi_2$ & $\varphi_3$ & $\varphi_1 \varphi_2$ & $\varphi_1 \varphi_3$ & $\varphi_2 \varphi_3$ & $\varphi_1^2$ & $\varphi_2^2$ & $\varphi_3^2$ \\
% \hline\hline
% A	&	0.02	&	0.37	&	0.77    &   -0.21   &   0.17    &   -       &   -   &   -0.06   &   -   &   -	    \\
% B	&	0.02	&	0.04	&	-       &   0.96    &   -       &   0.06    &   -   &   -0.03   &   -   &   -0.03	\\
% \hline
% \end{tabular}
% }
% \end{table}

==> nomenclature.tex <==
\section*{Nomenclature}

% \noindent $n$ : Number of nodes along feeder \\
\noindent $V_{\phi,k}$ : Voltage phasor at node $k$ on phase $\phi$ \\
\noindent $\mathbb{V}_{k}$ : Vector of voltage phasors at node $k$ \\
\noindent $y_{\phi,k}$ : Square magnitude of voltage at node $k$ on phase $\phi$ \\ %s.t. $Y_{\phi,k} = \left| V_{\phi,k} \right| ^2$ \\
\noindent $\mathbb{Y}_{k}$ : Vector of square magnitudes of voltage at node $k$ \\
\noindent $Z_{\phi \phi,jk}$ : Impedance of segment $(j,k)$ on phase $\phi$ \\
\noindent $Z_{\phi \psi,jk}$ : Impedance of segment $(j,k)$ between phases ($\phi,\psi$) \\
\noindent $\mathbb{Z}_{jk}$ : Impedance matrix of line segment $(j,k)$ \\
\noindent $I_{\phi,k}$ : Current phasor entering node $k$ on phase $\phi$ \\
\noindent $\mathbb{I}_{k}$ : Vector of current phasors entering node $k$ \\
\noindent $i_{\phi,k}$ : Load current of phase $\phi$ at node $k$ \\
\noindent $\mathbf{i}_{k}$ : Vector of load currents at node $k$ \\
\noindent $S_{\phi,k}$ : Phasor of complex power entering node $k$ on phase $\phi$ \\
\noindent $\mathbb{S}_{k}$ : Vector of complex power phasors entering node $k$ \\
\noindent $s_{\phi,k}$ : Complex load on phase $\phi$ at node $k$ \\
\noindent $\mathbf{s}_{k}$ : Vector of complex loads at node $k$ \\
\noindent $u_{\phi,k}$ : Inverter VAR dispatch on phase $\phi$ at node $k$

==> three_phase.tex <==
\section{Three-phase Power Flow Modeling}

Whereas the use of convex relaxations is well-applicable in single-phase networks, these are not yet robust enough for the more complex OPF formulations for unbalanced three-phase systems. Its development for three-phase networks~\cite{dallanese_distributed_2013} is hampered by issues of nondegeneracy and inexactness of the semidefinite relaxations~\cite{louca_nondegeneracy_2014}. In~\cite{sankur_optimal_2018,bolognani_fast_2016}, linear approximations of the unbalanced power flow are proposed to overcome these challenges and enable three-phase OPF for a broad range of conditions.
Here we adopt the modeling developed in~\cite{arnold_optimal_2016, sankur_linearized_2016,sankur_optimal_2018}, which can be seen as an adaptation of the \emph{DistFlow} model~\cite{baran_optimal_1989} to unbalanced circuits, coined the \emph{Dist3Flow} model. We restate part of the model's derivation here to provide sufficient intuition for its use in experiments.
% \subsection{Preliminaries}
% \label{subsec:preliminaries}
% \renewcommand{\arraystretch}{1.15}
% \setlength{\textfloatsep}{10pt}
% \begin{table}[t]
% \centering
% \caption{NOMENCLATURE}
% \begin{tabulary}{\linewidth}{LLL}
% 	\hline
% 	\hline
% % $\mathcal{P}_{n}$ && Set of phases that exist at node $n$ \\
% % \noindent $\mathcal{P}_{mn}$ & & Set of phases that exist on line $(m,n)$ \\
%   \noindent $V_{n}^{\phi}$ & & Voltage phasor at node $n$ on phase $\phi$ \\
%   \noindent $\mathbf{V}_{n}$ & & Vector of voltage phasors at node $n$ \\
%   \noindent $E_{n}^{\phi}$ & & Square magnitude of voltage at node $n$ on phase $\phi$ \\
%   \noindent $\mathbf{E}_{n}$ & & Vector of square magnitudes of voltage at node $n$ \\
%   $\theta_{n}^{\phi}$ & & Phase angle of voltage phasor at node $n$ on phase $\phi$ \\
%   \noindent $Z_{mn}^{\phi \phi}$ & & Impedance of segment $(m,n)$ on phase $\phi$ \\
%   \noindent $Z_{mn}^{\phi \psi}$ & & Impedance of segment $(m,n)$ between phases ($\phi,\psi$) \\
%   \noindent $\mathbf{Z}_{mn}$ & & Impedance matrix of line segment $(m,n)$ \\
%   \noindent $I_{mn}^{\phi}$ & & Current phasor on phase $\phi$ of segment $(m,n)$  \\
%   \noindent $\mathbf{I}_{mn}$ & & Vector of current phasors on all phases of segment $(m,n)$ \\
%   \noindent $i_{n}^{\phi}$ & & Nodal current of phase $\phi$ at node $n$ \\
%   \noindent $\mathbf{i}_{n}$ & & Vector of nodal currents at node $n$ \\
%   \noindent $S_{mn}^{\phi}$ & & Phasor of complex power on line $(m,n)$ on phase $\phi$ at node $n$ \\
%   \noindent $\mathbf{S}_{mn}$ & & Vector of complex power phasors on all phases of segment $(m,n)$ entering node $n$ \\
%   \noindent $s_{n}^{\phi}$ & & Complex nodal power on phase $\phi$ at node $n$ \\
%   \noindent $\mathbf{s}_{n}$ & & Vector of complex nodal powers for all phases at node $n$ \\
% %   \noindent $u_{n}^{\phi}$ & & Inverter real power dispatch on phase $\phi$ at node $n$ \\
% %   \noindent $v_{n}^{\phi}$ & & Inverter VAR dispatch on phase $\phi$ at node $n$ \\
%   \noindent $w_{n}^{\phi}$ & & Inverter complex dispatch on phase $\phi$ at node $n$ \\
%   \noindent $e_{n}^{\phi}$ & & Constant voltage reference for phase $\phi$ at node $n$ \\
%   \noindent $\mathbf{e}_{n}^{\phi}$ & & Vector of constant voltage references for node $n$ \\
%   \noindent $\left( \cdot \right)^{T}$ & & Transpose \\
%   \noindent $\left( \cdot \right)^{*}$ & & Complex conjugate \\
% %   \noindent $\left( \cdot \right)^{H}$ & & Complex conjugate transpose \\
%   \noindent $\mathcal{P}_{n}$ & & Set of phases that exist at node $n$ \\
%   \noindent $\mathcal{P}_{mn}$ & & Set of phases that exist on line $(m,n)$ \\
%   \hline
%   \hline
% \end{tabulary}
% \end{table}
% Let $\mathcal{T} = (\mathcal{N}, \mathcal{E})$ denote a graph representing an unbalanced distribution feeder, where $\mathcal{N}$ is the set of nodes of the feeder and $\mathcal{E}$ is the set of line segments. Nodes are indexed by $n = 0,1,\dots,N-1$, where $N$ is the order (number of nodes) of the distribution feeder, and node 0 denotes the feeder head (or substation). We treat node 0 as an infinite bus, decoupling interactions in the downstream distribution system from the rest of the grid. 
% While the substation voltage may evolve over time, we assume this evolution takes place independently of DER control actions in $\mathcal{T}$.
In this setting, each node and line segment can have up to three phases, labeled $a$, $b$, and $c$. Phases are referred to by the variables $\phi$ and $\psi$, where $\phi \in \{ a, b, c \}$, $\psi \in \{ a, b, c \}$. 
% If phase $\phi$ is present at node $m$, then at least one line connected to $m$ must contain phase $\phi$, such that:
% \begin{equation*}
% 	m \in \mathcal{N} \Rightarrow \mathcal{P}_{m} = \left( \cup_{l:(l,m) \in \mathcal{E}} \mathcal{P}_{lm} \right) \cup \left( \cup_{n:(m,n) \in \mathcal{E}} \mathcal{P}_{mn} \right)
% \end{equation*}
% \begin{equation*}
% m \in \mathcal{N} \Rightarrow \mathcal{P}_{m} = \cup_{n:(m,n) \in \mathcal{E}} \mathcal{P}_{mn}
% \end{equation*}
If line $(m,n)$ exists, its phases must be a subset of the phases present at both node $m$ and node $n$.
% , such that:
% \begin{equation*}
% (m,n) \in \mathcal{E} \Rightarrow \mathcal{P}_{mn} \subseteq \mathcal{P}_{m} \cap \mathcal{P}_{n}
% \end{equation*}
% However $\mathcal{P}_{m} \cap \mathcal{P}_{n} \neq \emptyset$ does not necessarily mean $\exists (m,n) \in \mathcal{E}$.

The current/voltage relationship for a three phase line $(m,n)$ between adjacent nodes $m$ and $n$ is captured by Kirchhoff's Voltage Laws (KVL) in its full \eqref{eq:KVLmn1}, and compact form \eqref{eq:KVLmn2}:
% \begin{equation}
\begin{gather}
	\begin{bmatrix}
		V_{m}^{a} \\ V_{m}^{b} \\ V_{m}^{c}
	\end{bmatrix}
	=
	\begin{bmatrix}
		V_{n}^{a} \\ V_{n}^{b} \\ V_{n}^{c}
	\end{bmatrix}
	+
	\begin{bmatrix}
		Z^{aa}_{mn} & Z^{ab}_{mn} & Z^{ac}_{mn} \\
		Z^{ba}_{mn} & Z^{bb}_{mn} & Z^{bc}_{mn} \\
		Z^{ca}_{mn} & Z^{cb}_{mn} & Z^{cc}_{mn}
	\end{bmatrix}
	\begin{bmatrix}
		I_{mn}^{a} \\ I_{mn}^{b} \\ I_{mn}^{c}
	\end{bmatrix}
    \label{eq:KVLmn1}
	\\
    \mathbf{V}_{m} = \mathbf{V}_{n} + \mathbf{Z}_{mn} \mathbf{I}_{mn}
    \label{eq:KVLmn2}
\end{gather}
% \label{eq:KVLmn}
% \end{equation}
Here, $Z^{\phi \psi}_{mn} = r^{\phi \psi}_{mn} + jx^{\phi \psi}_{mn}$ denotes the complex impedance of line $(m,n)$ across phases $\phi$ and $\psi$. 
% We have presented \eqref{eq:KVLmn1} and \eqref{eq:KVLmn2} where $\mathcal{P}_{mn} = \{ a, b, c\}$. 
% For lines with less than three phases ($\left| \mathcal{P}_{mn} \right| = 1$, or $\left| \mathcal{P}_{mn} \right| = 2$) \eqref{eq:KVLmn2} becomes:
% \begin{equation}
% 	\left[ \mathbf{V}_{m} \right]_{\mathcal{P}_{mn}}  = \left[ \mathbf{V}_{n} \right]_{\mathcal{P}_{mn}} + \left[ \mathbf{Z}_{mn} \right]_{\mathcal{P}_{mn},\mathcal{P}_{mn}} \left[ \mathbf{I}_{mn} \right]_{\mathcal{P}_{mn}}
%     \label{eq:KVLmn3}
% \end{equation}
% \todo[inline]{Need to define notation for $\left[ \cdot \right]_{\mathcal{P}_{mn}}$. Typo in $\left[ \mathbf{Z}_{mn} \right]_{\mathcal{P}_{mn},\mathcal{P}_{mn}}$? (double subscript) - Defined in Dall'Anese paper, double subscript is correct. The commented stuff below defines it using their almost exact wording.}
% \noindent where for a vector $\mathbf{A}$, $\left[ \mathbf{A} \right]_{\mathcal{P}}$ denotes a $\left| \mathcal{P} \right| \times 1$ sub-vector containing entries of $\mathbf{A}$ indexed by $\mathcal{P}$, and for a matrix $\mathbf{B}$, $\left[ \mathbf{B} \right]_{\mathcal{P}_{1},\mathcal{P}_{2}}$ denotes a $\left| \mathcal{P}_{1} \right| \times \left| \mathcal{P}_{2} \right|$ sub-matrix with rows of $\mathbf{B}$ indexed by $\mathcal{P}_{1}$ and columns of $\mathbf{B}$ indexed by $\mathcal{P}_{2}$. Here, we have reused the notation and description from \cite{dall2013distributed}. If equations are to be indexed by $\mathcal{P}_{mn}$, they should be indexed as in \eqref{eq:KVLmn3}, where vectors are indexed by $\mathcal{P}_{mn}$ and
% \noindent by employing the same indexing notation as in \cite{dall2013distributed}, whereby rows of \eqref{eq:KVLmn3} and columns of $\mathbf{Z}_{mn}$ corresponding to $\phi \notin \mathcal{P}_{mn}$ are removed. To give two examples, if $\mathcal{P}_{mn} = \left\{ a \right\}$, then \eqref{eq:KVLmn3} for line $(m,n)$ is $V_{m}^{a} = V_{n}^{a} + Z_{mn}^{aa} I_{mn}^{a}$ and if $\mathcal{P}_{mn} = \left\{ a , c \right\}$ then \eqref{eq:KVLmn3} for line $(m,n)$ becomes:
% \begin{equation*}
% 	\begin{bmatrix}
% 		V_{m}^{a} \\ V_{m}^{c}
% 	\end{bmatrix}
% 	=
% 	\begin{bmatrix}
% 		V_{n}^{a} \\ V_{n}^{c}
% 	\end{bmatrix}
% 	+
% 	\begin{bmatrix}
% 		Z^{aa}_{mn} & Z^{ac}_{mn} \\
% 		Z^{ca}_{mn} & Z^{cc}_{mn}
% 	\end{bmatrix}
% 	\begin{bmatrix}
% 		I_{mn}^{a} \\ I_{mn}^{c}
% 	\end{bmatrix}
% \end{equation*}
%
% \noindent Additionally, if $\phi \notin \mathcal{P}_{n}$ we define $V_{n}^{\phi} = 0$. If $\phi \notin \mathcal{P}_{mn}$, we define $I_{mn}^{\phi} = 0$, and $Z_{mn}^{\phi \psi} = Z_{mn}^{\psi \phi} = 0 \qq \forall \psi \in \{ a, b, c \}$.
% \todo[inline]{I pushed this sentence back - to double check: is this correct? Is this what Emilio does?}
% \todo[inline]{Dall'Anese completely omits these values. We can omit V}
%
% Kirchoff's Current law at node $m$ is given in its full \eqref{eq:KCLm1} and compact \eqref{eq:KCLm2} forms:
% % \begin{equation}
% \begin{gather}
% 	\sum_{l:(l,m) \in \mathcal{E}}
% 	\begin{bmatrix}
% 		I_{lm}^{a} \\ I_{lm}^{b} \\ I_{lm}^{c}
% 	\end{bmatrix}
% 	=
%     \begin{bmatrix}
% 		i_{m}^{a} \\ i_{m}^{b} \\ i_{m}^{c}
% 	\end{bmatrix}
%     +
%     \sum_{n:(m,n) \in \mathcal{E}}
% 	\begin{bmatrix}
% 		I_{mn}^{a} \\ I_{mn}^{b} \\ I_{mn}^{c}
% 	\end{bmatrix}
%     \label{eq:KCLm1}
% 	\\
% 	\sum_{l:(l,m) \in \mathcal{E}} \mathbf{I}_{lm} = \mathbf{i}_{m} + \sum_{n:(m,n) \in \mathcal{E}} \mathbf{I}_{mn}
%     \label{eq:KCLm2}
% \end{gather}
% % \label{eq:KCLm}
% % \end{equation}
%
% % $\mathbf{I}_{mn} = \left[I_{mn}^{a} \text{, } I_{mn}^{b} \text{, } I_{mn}^{c} \right]^{T}$
% % $\mathbf{i}_{mn} = \left[i_{mn}^{a} \text{, } i_{mn}^{b} \text{, } i_{mn}^{c} \right]^{T}$
%
% \noindent We assume a complex load is served at each node, where the load on a phase $s_{n}^{\phi} = V_{n}^{\phi} {\left( i_{n}^{\phi} \right)}^{*} \in \mathbf{C}$ is defined as:
% \begin{equation}
% 	s_{n}^{\phi} \left( V_{n}^{\phi} \right) = \left(A_{PQ,n}^{\phi} + A_{Z,n}^{\phi} \left| V_{n}^{\phi} \right|^{2} \right) d_{n}^{\phi} + w_{n}^{\phi} - j y_{n}^{\phi}
%     \label{eq:sV}
% \end{equation}
% \noindent where $d_{n}^{\phi}$ is the voltage dependent complex demand, $A_{PQ,n}^{\phi} + A_{Z,n}^{\phi} = 1$, $w_{n}^{\phi} = u_{n}^{\phi} + j v_{n}^{\phi}$ denotes the complex DER dispatch, and $y_{n}^{\phi}$ denotes capacitance, with $\phi \in \mathcal{P}_{n}$. The vector of complex loads at node $n$ is $\mathbf{s}_{n} = \left[ s_{n}^{a}, \qq s_{n}^{b}, \qq s_{n}^{c} \right]^{T}$.
% % $\mathbf{s}_{n} = \begin{bmatrix} s_{n}^{a} & s_{n}^{b} & s_{n}^{c} \end{bmatrix}^{T}$
%
% Throughout this work, we use the symbol $\circ$ to represent the Hadamard Product (HP) of two matrices (or vectors) of the same dimension, also known of the element-wise product, such that:
% \begin{equation*}
% 	C = A \circ B = B \circ A \Rightarrow C_{ij} = A_{ij} B_{ij} = B_{ij} A_{ij}
%     \label{eq:hadamard}
% \end{equation*}
%
% \noindent where $i$ indicates the row and $j$ indicates the column of the vector or matrix.
%
%
% \subsection{Power and Losses}
% \label{subsec:power}
%
% We now derive complex power and loss terms at a node $m \in \mathcal{N}$. This derivation follows that of \cite{gan2014convex} and \cite{robbins2016optimal} for three phases systems. Our derivation arrives at the same result as in \cite{gan2014convex}, but with different nomenclature and method. %This derivation will be presented assuming a three phase node and lines. For systems with nodes and lines with less than three phases, all equations should be indexed appropriately.
%
% To start, we take the HP of $\mathbf{V}_{m}$ and the complex conjugate (non-transposed) of \eqref{eq:KCLm2}:
% \begin{equation}
%     \sum_{l:(l,m) \in \mathcal{E}} \mathbf{V}_{m} \circ \mathbf{I}_{lm}^{*} = \mathbf{V}_{m} \circ \mathbf{i}_{m}^{*} + \sum_{n:(m,n) \in \mathcal{E}} \mathbf{V}_{m} \circ \mathbf{I}_{mn}^{*}
%     \label{eq:power01}
% \end{equation}
%
% \noindent The $\mathbf{V}_{m}$ term inside the summation on the RHS is  substituted using \eqref{eq:KVLmn2}:
% \begin{equation}
% \begin{aligned}
%     \sum_{l:(l,m) \in \mathcal{E}} \mathbf{V}_{m} & \circ \mathbf{I}_{lm}^{*} = \mathbf{V}_{m} \circ \mathbf{i}_{m}^{*} + \ldots \\
%     & \sum_{n:(m,n) \in \mathcal{E}}  \mathbf{V}_{n} \circ \mathbf{I}_{mn}^{*} + \left( \mathbf{Z}_{mn} \mathbf{I}_{mn} \right) \circ \mathbf{I}_{mn}^{*}
% \end{aligned}
% \label{eq:power02}
% \end{equation}

\noindent Next, we define the per phase complex power as $\mathbf{S}_{mn}^{\phi} = \mathbf{V}_{n}^{\phi} \left( \mathbf{I}_{mn}^{\phi} \right)^{*}$
%we define $\mathbf{S}_{lm} = \mathbf{V}_{m} \circ \mathbf{I}_{lm}^{*}$ and $\mathbf{S}_{mn} = \mathbf{V}_{n} \circ \mathbf{I}_{mn}^{*}$, where $\mathbf{S}_{lm}$ is the power from node $l$ to node $m$ at node $m$m and $\mathbf{S}_{mn}$ is the power from node $m$ to node $n$ at node $n$.
, and the $3 \times 1$ vector of complex power phasors $\mathbf{S}_{mn} = \mathbf{V}_{n} \circ \mathbf{I}_{mn}^{*}$ where $\mathbf{S}_{mn}$ is the power from node $m$ to node $n$ at node $n$.
\begin{equation}
    \sum_{l:(l,m) \in \mathcal{E}} \mathbf{S}_{lm} = \mathbf{s}_{m} + \sum_{n:(m,n) \in \mathcal{E}} \mathbf{S}_{mn} + \mathbf{L}_{mn}
    \label{eq:power03}
\end{equation}

The term $\mathbf{L}_{mn} \in \mathbf{C}^{3 \times 1}$ is a nonlinear and non-convex loss term. As in \cite{gan_convex_2014} and \cite{baran_optimal_1989}, we assume that losses are negligible compared to line flows, so that $\left| L_{mn}^{\phi} \right| \ll \left| S_{mn}^{\phi} \right| \ \forall (m,n) \in \mathcal{E}$. Thus, we neglect line losses, linearizing \eqref{eq:power03} into \eqref{eq:power04}.
\begin{equation}
    \sum_{l:(l,m) \in \mathcal{E}} \mathbf{S}_{lm} \approx \mathbf{s}_{m} + \sum_{n:(m,n) \in \mathcal{E}} \mathbf{S}_{mn}
    \label{eq:power04}
\end{equation}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% In this section, we introduce and define several important parameters, approximations, relationships and equations. The constant $\alpha$, extensively used in the study and analysis of power systems, is defined by (\eqref{eq:def_alpha}).

% \begin{equation}
% 	\alpha = 1 \angle 120 \degree \quad \alpha^{2} = 1 \angle 240 \degree
%     \label{eq:def_alpha}
% \end{equation}

% In (\eqref{eq:VaVbVc}), we introduce an approximation for the quotient of two different phasee voltage phasors at a node. We assume that the magnitude of the phasors for each phase are roughly equivalent at each node. Furthermore, we assume that the phase angle difference is $\pm 120 \degree$ as appropriate. These assumptions are reflected in (\eqref{eq:VaVbVc}).

% \begin{equation}
% 	V_{a,k} V_{b,k}^{-1} \approx \alpha \quad V_{b,k} V_{c,k}^{-1} \approx \alpha \quad V_{a,k} V_{c,k}^{-1} \approx \alpha^{2}
%     \label{eq:VaVbVc}
% \end{equation}

% A vector of general values for the three phases at a node is defined by (\eqref{eq:def_Xk}). Bold font ($\mathbb{X}$) indicates a vector or matrix, and the subscript $k$ indicates the node. Normal font ($X$) indicates a value at a particular phase. The first subscript indicates the phase, with $\phi$ being a general phase, and $a,b,c$ the actual phase. The second subscript $k$, if present, indicates the node of the individual value or vector.

% \begin{equation}
% 	\mathbb{X}_{k}
%     =
%     \begin{bmatrix}
%     X_{a,k} \\
%     X_{b,k} \\
%     X_{c,k} \\
%     \end{bmatrix}
%     =
%     \begin{bmatrix}
%     X_{a} \\
%     X_{b} \\
%     X_{c} \\
%     \end{bmatrix}_{k}
%     \label{eq:def_Xk}
% \end{equation}

% The power entering a node on a phase is defined as the phase voltage at the node multiplied by the complex conjugate of the phase current entering the node, as in (\eqref{eq:def_Sk}). 

% \begin{equation}
% 	S_{\phi,k} = V_{\phi,k} I_{\phi,k}^{*}
%     \label{eq:def_Sk}
% \end{equation}

% The squared magnitude of a voltage phasor is given by (\eqref{eq:def_Yk}).

% \begin{equation}
% 	y_{\phi,k} = \left| V_{\phi,k} \right|^2 = V_{\phi,k} V_{\phi,k}^*
%     \label{eq:def_Yk}
% \end{equation}

% Kirchoff's Voltage Law for a three phase line between two nodes is given by (\eqref{eq:kvl_3phase}), and is represented in its compact and expanded form. In all equations we assume node $k-1$ is immediately upstream (toward the feeder head) of node $k$.

% % \begin{equation}
% % \begin{gathered}
% % 	\mathbb{V}_{k-1} = \mathbb{V}_{k} + \mathbb{Z}_{k} \mathbb{I}_{k} \\
% %     \begin{bmatrix}
% %   		V_{a} \\
% %   		V_{b} \\
% %   		V_{c}
% %   	\end{bmatrix}_{k-1}
% %   	=
% %   	\begin{bmatrix}
% %   		V_{a} \\
% %   		V_{b} \\
% %   		V_{c}
% %   	\end{bmatrix}_{k}
% %   	+
% %   	\begin{bmatrix}
% %   		Z_{aa} & Z_{ab} & Z_{ac} \\
% %   		Z_{ba} & Z_{bb} & Z_{bc} \\
% %   		Z_{ca} & Z_{cb} & Z_{cc}
% %   	\end{bmatrix}_k
% %   	\begin{bmatrix}
% %   		I_{a} \\
% %   		I_{b} \\
% %   		I_{c}
% %   	\end{bmatrix}_k
% % \end{gathered}
% % \label{eq:kvl_3phase}
% % \end{equation}

% % \begin{figure}[t]
% % 	\centering
% % 	\includegraphics[width=0.5\textwidth, clip, trim = 2.875in 2.875in 2.375in 2.125in]{kvl.pdf}
% %     \caption{Nodes $k-1$ and $k$ with line impedances and power entering the phases at node $k$ shown.}
% % 	\label{fig:kvl_3phase}
% % \end{figure}


% % \begin{equation}
% % 	y_{\phi,k-1} = f \left( \mathbb{Y}_{k} , \mathbb{P}_{k}, \mathbb{Q}_{k} \right)
% % \end{equation}

% We start by considering (\eqref{eq:kvl_3phase}), and right multiply each side by their complex conjugate as in (\eqref{eq:mag_1}). Though this results in $3 \times 3$ matrices in (\eqref{eq:mag_1}), we are only interested in the entries on the diagonals of each matrix, which represent each row of the (\eqref{eq:kvl_3phase}) multiplied by its complex conjugate. Adding complex conjugates results in the second row of (\eqref{eq:mag_1}).

% % \setlength{\abovedisplayskip}{-5pt} \setlength{\abovedisplayshortskip}{-5pt}
% % \setlength{\belowdisplayskip}{-5pt} \setlength{\belowdisplayshortskip}{-5pt}

% \begin{equation}
% \begin{aligned}
% 	\mathbb{V}_{j} \mathbb{V}_{j}^*  & =  \mathbb{V}_{k} \mathbb{V}_{k}^* + \mathbb{Z}_{k} \mathbb{I}_{k} \mathbb{V}_{k}^* + \mathbb{V}_{k} \mathbb{I}_{k}^{*} \mathbb{Z}_{k}^{*} + \mathbb{Z}_{k} \mathbb{I}_{k} \mathbb{I}_{k}^{*} \mathbb{Z}_{k}^{*} \\
%     & = \mathbb{V}_{k} \mathbb{V}_{k}^* + 2 \Re \left\{\mathbb{V}_{k} \mathbb{I}_{k}^{*} \mathbb{Z}_{k}^{*} \right\} + \mathbb{Z}_{k} \mathbb{I}_{k} \mathbb{I}_{k}^{*} \mathbb{Z}_{k}^{*}
% \end{aligned}
% \label{eq:mag_1}
% \end{equation}

% Voltage constraints dictate that feeder node voltage be within a $\pm 5 \%$ range of 1 pu, such that $0.95 \le \left| V_{\phi,k} \right| \le 1.05 \quad \forall \phi, k$. The magnitudes of line and mutual impedances are generally much smaller than 1, the magnitudes of current phasors are generally smaller than $1$. Normal values of impedance and current magnitude are such that $\left| Z_{\phi\phi} \right| \le 0.1$, $\left| Z_{\phi\psi} \right| \le 0.1$, and $\left| I_{\phi} \right| \le 0.5$. Thus approximate magnitudes of elements of $\mathbb{V}_{k} \mathbb{I}_{k}^{*} \mathbb{Z}_{k}^{*}$ and $\mathbb{Z}_{k} \mathbb{I}_{k} \mathbb{I}_{k}^{*} \mathbb{Z}_{k}^{*}$ are shown the first and second row of (\eqref{eq:mag_approx}), respectively.

% \begin{equation}
% \begin{aligned}
% 	& \left| V_{a,k} Z_{aa,k}^* I_{a,k}^* \right| = \left| V_{a,k} \right| \left| Z_{aa,k} \right| \left| I_{a,k} \right| \approx 0.01 \\
%     & \left| Z_{aa,k} I_{a,k} Z_{ab,k}^* I_{b,k}^* \right| = \left| Z_{aa,k} \right| \left| I_{a,k} \right| \left| Z_{ab,k} \right| \left| I_{b,k} \right| \approx 0.0001
% \end{aligned}
% \label{eq:mag_approx}
% \end{equation}

% By (\eqref{eq:mag_approx}), higher order terms such as $\left| Z_{aa,k} I_{a,k} \right|^2$ and $Z_{aa,k} I_{a,k} Z_{ab,k}^* I_{b,k}^*$ which are components of $\mathbb{Z}_{k} \mathbb{I}_{k} \mathbb{I}_{k}^* \mathbb{Z}_{k}^*$ are of negligible magnitude compared to other terms such as $V_{a,k} Z_{aa,k}^* I_{a,k}^*$, which is a component of $\mathbb{V}_{k} \mathbb{I}_{k}^* \mathbb{Z}_{k}^*$. Treating higher order terms of $\mathbb{Z}_{k} \mathbb{I}_{k} \mathbb{I}_{k}^{*} \mathbb{Z}_{k}^{*}$ as negligible simplifies (\eqref{eq:mag_1}) to (\eqref{eq:mag_2}).

% \begin{equation}
% 	\mathbb{V}_{j} \mathbb{V}_{j}^{*} = \mathbb{V}_{k} \mathbb{V}_{k}^{*} + 2 \Re \left\{ \mathbb{V}_{k} \mathbb{I}_{k}^{*} \mathbb{Z}_{k}^{*} \right\}
%     \label{eq:mag_2}
% \end{equation}

% We take advantage (\eqref{eq:def_Sk}) to replace the current phasors in (\eqref{eq:mag_2}), as in (\eqref{eq:mag_3}).

% \begin{equation}
% 	\begin{aligned}
% 		\mathbb{V}_{j} & \mathbb{V}_{j}^{*} = \mathbb{V}_{k} \mathbb{V}_{k}^{*} + \ldots \\
%     	& 2 \Re \left\{ \mathbb{V}_{k}
%     	\begin{bmatrix}
%     		S_{a} V_{a}^{-1} & S_{b} V_{b}^{-1} & S_{c} V_{c}^{-1}
%     	\end{bmatrix}_k
%     	\mathbb{Z}_{jk}^* \right\}
%     \end{aligned}
%     \label{eq:mag_3}
% \end{equation}

% \begin{equation}
% 		\mathbb{V}_{j} \mathbb{V}_{j}^{*} = \mathbb{V}_{k} \mathbb{V}_{k}^{*} +
%     	2 \Re \left\{ \mathbb{V}_{k}
%     	\begin{bmatrix}
%     		S_{a} V_{a}^{-1} & S_{b} V_{b}^{-1} & S_{c} V_{c}^{-1}
%     	\end{bmatrix}_k
%     	\mathbb{Z}_{jk}^* \right\}
%     \label{eq:mag_3}
% \end{equation}

% Multiplying the first two matrices results in (\eqref{eq:mag_4}), and using (\eqref{eq:VaVbVc}) gives (\eqref{eq:mag_5}).

% % \begin{equation}
% % 	\mathbb{Y}_{k-1} = \mathbb{Y}_{k} + 2 \Re \left\{
% %     \begin{bmatrix}
% %     	S_{a,k} & V_{a,k} S_{b,k} V_{b,k}^{-1} & V_{a,k} S_{c,k} V_{c,k}^{-1} \\
% %     	V_{b,k} S_{a,k} V_{a,k}^{-1} & S_{b,k} & V_{b,k} S_{c,k} V_{c,k}^{-1} \\
% %     	V_{c,k} S_{a,k} V_{a,k}^{-1} & V_{c,k} S_{b,k} V_{b,k}^{-1} & S_{c,k}
% %     \end{bmatrix}
% %     \mathbb{Z}_{k}^* \right\} \\
% %     \label{eq:mag_4}
% % \end{equation}

% \begin{equation}
% 	\begin{aligned}
% 		\mathbb{V}_{j} & \mathbb{V}_{j}^{*} = \mathbb{V}_{k} \mathbb{V}_{k}^{*} + \ldots \\
%     	& 2 \Re \left\{
%     	\begin{bmatrix}
%     		S_{a} & V_{a} S_{b} V_{b}^{-1} & V_{a} S_{c} V_{c}^{-1} \\
%     		V_{b} S_{a} V_{a}^{-1} & S_{b} & V_{b} S_{c} V_{c}^{-1} \\
%     		V_{c} S_{a} V_{a}^{-1} & V_{c} S_{b} V_{b}^{-1} & S_{c}
%     	\end{bmatrix}_k
%     	\mathbb{Z}_{jk}^* \right\}
%     \end{aligned}
%     \label{eq:mag_4}
% \end{equation}
	
% \begin{equation}
% 	\mathbb{V}_{j} \mathbb{V}_{j}^{*} = \mathbb{V}_{k} \mathbb{V}_{k}^{*} + 2 \Re \left\{
%     \begin{bmatrix}
%     	S_{a} & \alpha S_{b} & \alpha^{2} S_{c} \\
%     	\alpha^{2} S_{a} & S_{b} & \alpha S_{c} \\
%     	\alpha S_{a} & \alpha^{2} S_{b} & S_{c}
%     \end{bmatrix}_k
%     \mathbb{Z}_{jk}^* \right\}
%     \label{eq:mag_5}
% \end{equation}

% By multiplying the vectors by their complex conjugate to obtain matrices, multiplying the two matrices inside the $\Re$ operator together, and collecting the diagonal elements of all matrices and placing them into vectors gives (\eqref{eq:mag_6}). Here we use define the vector of phase square voltage magnitude as $\mathbb{Y}_{k} = \begin{bmatrix} y_{a,k} & y_{b,k} & y_{c,k} \end{bmatrix}^{T}$.

% \begin{equation}
% 	\mathbb{Y}_{j} = \mathbb{Y}_{k} + 2 \Re \left\{
%     \begin{bmatrix}
%     	Z_{aa}^{*} S_{a}  + \alpha Z_{ab}^{*} S_{b}  + \alpha^{2} Z_{ac}^{*} S_{c} \\
%     	\alpha^{2} Z_{ba}^{*} S_{a} + Z_{bb}^{*} S_{b} + \alpha Z_{bc}^{*} S_{c} \\
%     	\alpha Z_{ca}^{*} S_{a} + \alpha^{2} Z_{cb}^{*} S_{b} + Z_{cc}^{*} S_{c}
%     \end{bmatrix}_k
% 	\right\}
%     \label{eq:mag_6}
% \end{equation}

% The matrix inside the $\Re$ operator can be broken into a $3 \times 3$ matrix and a vector of node complex power, as in (\eqref{eq:mag_7}).

% \begin{equation}
% 	\mathbb{Y}_{j}= \mathbb{Y}_{k} + 2 \Re \left\{
%     \begin{bmatrix}
%     	Z_{aa}^{*} & \alpha Z_{ab}^{*} & \alpha^{2} Z_{ac}^{*} \\
%     	\alpha^{2} Z_{ba}^{*} & Z_{bb}^{*} & \alpha Z_{bc}^{*} \\
%     	\alpha Z_{ca}^{*} & \alpha^{2} Z_{cb}^{*} & Z_{cc}^{*}
%     \end{bmatrix}_{jk}
%     \begin{bmatrix}
%     	S_{a} \\ S_{b} \\ S_{c}
%     \end{bmatrix}_{jk}
% 	\right\}
%     \label{eq:mag_7}
% \end{equation}

% Expanding the impedance matrix entries as $Z_{\phi \psi,k} = r_{\phi, \psi,k} + j x_{\phi, \psi,k}$, the complex power as $S_{\phi,k} = P_{\phi,k} + j Q_{\phi,k}$, the constant $\alpha$ as  $\alpha = \frac{1}{2}(1 + j \sqrt{3})$, and $\alpha^2 = \frac{1}{2}(1 - j \sqrt{3})$, it can be shown that (\eqref{eq:mag_7}) simplifies to (\eqref{eq:mag_8}).

% \begin{equation}
% \begin{gathered}
% 	\mathbb{Y}_{j} = \mathbb{Y}_{k} + \mathbb{M}_{jk}^{P} \mathbb{P}_{k} + \mathbb{M}_{jk}^{Q} \mathbb{Q}_{k} \\
% 	\mathbb{M}_{jk}^{P} =
% 	\begin{bmatrix}
% 		2 r_{aa} & -r_{ab} + \sqrt{3} x_{ab} & -r_{ac} - \sqrt{3} x_{ac} \\
% 		-r_{ba} - \sqrt{3}x_{ba} & 2 r_{bb} & -r_{bc} + \sqrt{3}x_{bc} \\
% 		-r_{ca} + \sqrt{3}x_{ca} & -r_{cb} - \sqrt{3}x_{cb} & 2 r_{cc}
% 	\end{bmatrix}_{jk} \\
% 	\mathbb{M}_{jk}^{Q} =
% 	\begin{bmatrix}
% 		2 x_{aa} & -\sqrt{3} r_{ab} - x_{ab} & \sqrt{3} r_{ac} - x_{ac} \\
% 		\sqrt{3} r_{ba} - x_{ba} & 2 x_{bb} & -\sqrt{3} r_{bc} - x_{bc} \\
% 		-\sqrt{3} r_{ca} - x_{ca} & \sqrt{3} r_{cb} - x_{cb} & 2 x_{cc}
% 	\end{bmatrix}_{jk}	\\
% \end{gathered}
% \label{eq:mag_8}
% \end{equation}

% Equation (\eqref{eq:mag_8}) provides a linear equation in real and reactive power, if the line and mutual impedance values are treated as parameters. As (\eqref{eq:mag_8}) is linear, it does not affect the convexity of a system of equations. Using (\eqref{eq:mag_8}) to propagate voltage magnitude throughout a feeder provides a series of linear relations for all nodes, dependent on the power entering each node.

% It is clear that using (\eqref{eq:kvl_3phase}) to propagate voltage throughout the feeder would lead to a system of nonlinear equations to find the voltage magnitudes. This approximation bypasses these nonlinearities and does not affect convexity.

% \begin{equation}
% 	\mathbb{Y}_{k-1} = \mathbb{Y}_{k} + M_{k}^{P} P_{k} + M_{k}^{Q} Q_{k}
%     \label{eq:mag_8}
% \end{equation}

% \begin{equation}
% M_{k}^{P} =
% \begin{bmatrix}
% 2 r_{aa,k} & -r_{ab,k} + \sqrt{3} x_{ab,k} & -r_{ac,k} - \sqrt{3} x_{ac,k} \\
% -r_{ba,k} - \sqrt{3}x_{ba,k} & 2 r_{bb,k} & -r_{bc,k} + \sqrt{3}x_{bc,k} \\
% -r_{ca,k} + \sqrt{3}x_{ca,k} & -r_{cb,k} - \sqrt{3}x_{cb,k} & 2 r_{cc,k}
% \end{bmatrix}
% \label{eq:MP}
% \end{equation}

% \begin{equation}
% M_{k}^{P} =
% \begin{bmatrix}
% 2 r_{aa} & -r_{ab} + \sqrt{3} x_{ab} & -r_{ac} - \sqrt{3} x_{ac} \\
% -r_{ba} - \sqrt{3}x_{ba} & 2 r_{bb} & -r_{bc} + \sqrt{3}x_{bc} \\
% -r_{ca} + \sqrt{3}x_{ca} & -r_{cb} - \sqrt{3}x_{cb} & 2 r_{cc}
% \end{bmatrix}_k
% \label{eq:MP}
% \end{equation}

% \begin{equation}
% M_{k}^{Q} =
% \begin{bmatrix}
% 2 x_{aa,k} & -\sqrt{3} r_{ab,k} - x_{ab,k} & \sqrt{3} r_{ac,k} - x_{ac,k} \\
% \sqrt{3} r_{ba,k} - x_{ba,k} & 2 x_{bb,k} & -\sqrt{3} r_{bc,k} - x_{bc,k} \\
% -\sqrt{3} r_{ca,k} - x_{ca,k} & \sqrt{3} r_{cb,k} - x_{cb,k} & 2 x_{cc,k}
% \end{bmatrix}
% \label{eq:MQ}
% \end{equation}

% \begin{equation}
% M_{k}^{Q} =
% \begin{bmatrix}
% 2 x_{aa} & -\sqrt{3} r_{ab} - x_{ab} & \sqrt{3} r_{ac} - x_{ac} \\
% \sqrt{3} r_{ba} - x_{ba} & 2 x_{bb} & -\sqrt{3} r_{bc} - x_{bc} \\
% -\sqrt{3} r_{ca} - x_{ca} & \sqrt{3} r_{cb} - x_{cb} & 2 x_{cc}
% \end{bmatrix}_k
% \label{eq:MQ}
% \end{equation}

% \subsection{Magnitude Equations}
% \label{subsec:magnitude}

% In this section, we present a derivation for squared voltage magnitudes and complex multiphase power for unbalanced systems. This section follows derivations in \cite{gan2014convex} and \cite{robbins2016optimal}, however we present it in this work to keep a uniform nomenclature with the next section, to motivate the extension of the model to consider voltage angles in the following section, and to highlight a common structure shared between the voltage magnitude/complex power flow and voltage angle/complex power flow relationships.

% The reader should note that here we present the derivation for a line with three phases  where $\mathcal{P}_{mn} = \{ a, b, c \}$. For lines with less than three phases ($\left| \mathcal{P}_{mn} \right| = 1$ or $\left| \mathcal{P}_{mn} \right| = 2$), all equations should be indexed by $\mathcal{P}_{mn}$ as \eqref{eq:KVLmn3} is.

% To start, we consider a line $(m,n) \in \mathcal{E}$, and take the Hadamard Product of \eqref{eq:KVLmn2} and its (non-transposed) complex conjugate:
% \begin{equation}
% 	\mathbf{V}_{m} \circ \mathbf{V}_{m}^{*} = \left( \mathbf{V}_{n} + \mathbf{Z}_{mn} \mathbf{I}_{mn} \right) \circ \left( \mathbf{V}_{n} + \mathbf{Z}_{mn} \mathbf{I}_{mn} \right)^{*}
%     \label{eq:mag01}
% \end{equation}

% \noindent This can be rewritten by distributing the terms on the RHS:
% \begin{equation}
% \begin{aligned}
% 	\mathbf{V}_{m} & \circ \mathbf{V}_{m}^{*} = \mathbf{V}_{n} \circ \mathbf{V}_{n}^{*} + \mathbf{V}_{n} \circ  \left( \mathbf{Z}_{mn} \mathbf{I}_{mn} \right)^{*} + \ldots \\
%     & \left( \mathbf{Z}_{mn} \mathbf{I}_{mn} \right) \circ \mathbf{V}_{n}^{*} + \left( \mathbf{Z}_{mn} \mathbf{I}_{mn} \right) \circ \left( \mathbf{Z}_{mn} \mathbf{I}_{mn} \right)^{*}    
% \end{aligned}
% \label{eq:mag02}
% \end{equation}

\noindent Now, we define the real scalar $y_{m}^{\phi} = \left| V_{m}^{\phi} \right|^{2} = V_{m}^{\phi} (V_{m}^{\phi})^{*}$, the $3 \times 1$  real vector $\mathbf{y}_{m} = \left[ y_{m}^{a} , \ y_{m}^{b} , \ y_{m}^{c} \right]^{T} = \mathbf{V}_{m} \circ \mathbf{V}_{m}^{*}$.
With these definitions, \cite{sankur_optimal_2018} derives the following equations that govern the relationship between squared voltage magnitudes and complex power flow across line $(m,n)$:
% \begin{equation}
% % \begin{aligned}
% 	\mathbf{Y}_{m} = \mathbf{Y}_{n} +
% 	2 \Re \left\{ \left( \mathbf{Z}_{mn} \mathbf{I}_{mn} \right)^{*} \circ \mathbf{V}_{n} \right\} + \mathbf{H}_{mn} \,,
% % \end{aligned}
% 	\label{eq:mag03}
% \end{equation}
% Expanding the terms inside the real operators yields:
% \begin{equation}
% \begin{aligned}
% 	\mathbf{E}_{m} & = \mathbf{E}_{n} + \mathbf{H}_{mn} + \ldots \\
% 	& 2 \Re
%     \left\{
%     \begin{bmatrix}
%     	V_{n}^{a} \left( Z_{mn}^{aa} I_{mn}^{a} + Z_{mn}^{ab} I_{mn}^{b} + Z_{mn}^{ac} I_{mn}^{c} \right)^{*} \\
%         V_{n}^{b} \left( Z_{mn}^{ba} I_{mn}^{a} + Z_{mn}^{bb} I_{mn}^{b} + Z_{mn}^{bc} I_{mn}^{c} \right)^{*} \\
%         V_{n}^{c} \left( Z_{mn}^{ca} I_{mn}^{a} + Z_{mn}^{cb} I_{mn}^{b} + Z_{mn}^{cc} I_{mn}^{c} \right)^{*}
%     \end{bmatrix}
%     \right\} 
% \end{aligned}
% \end{equation}
% 
% \begin{equation}
% \begin{aligned}
% 	& \mathbf{E}_{m} = \mathbf{E}_{n} + \mathbf{H}_{mn} + \ldots \\
% 	& 2 \Re
%     \left\{
%     \begin{bmatrix}
%     	Z_{mn}^{aa} I_{mn}^{a} + Z_{mn}^{ab} I_{mn}^{b} + Z_{mn}^{ac} I_{mn}^{c} \\
%         Z_{mn}^{ba} I_{mn}^{a} + Z_{mn}^{bb} I_{mn}^{b} + Z_{mn}^{bc} I_{mn}^{c} \\
%         Z_{mn}^{ca} I_{mn}^{a} + Z_{mn}^{cb} I_{mn}^{b} + Z_{mn}^{cc} I_{mn}^{c}
%     \end{bmatrix}^{*}
%     \circ
%     \begin{bmatrix}
%     	V_{n}^{a} \\ V_{n}^{b} \\ V_{n}^{c}
%     \end{bmatrix}
%     \right\} 
% \end{aligned}
% \end{equation}
% 
% At this point, we focus on the terms inside the real operator ($\Re$) for clarity of presentation. %We expand $\left( \mathbf{Z}_{mn} \mathbf{I}_{mn} \right)^{*} \circ \mathbf{V}_{n}$ to obtain:
% \begin{equation}
% \begin{aligned}
% 	& \left( \mathbf{Z}_{mn} \mathbf{I}_{mn} \right)^{*} \circ \mathbf{V}_{n} = \ldots \\
%     & \quad
%     \begin{bmatrix}
%     	V_{n}^{a} \left( Z_{mn}^{aa} I_{mn}^{a} + Z_{mn}^{ab} I_{mn}^{b} + Z_{mn}^{ac} I_{mn}^{c} \right)^{*} \\
%         V_{n}^{b} \left( Z_{mn}^{ba} I_{mn}^{a} + Z_{mn}^{bb} I_{mn}^{b} + Z_{mn}^{bc} I_{mn}^{c} \right)^{*} \\
%         V_{n}^{c} \left( Z_{mn}^{ca} I_{mn}^{a} + Z_{mn}^{cb} I_{mn}^{b} + Z_{mn}^{cc} I_{mn}^{c} \right)^{*}
%     \end{bmatrix}
% \end{aligned}
% \label{eq:mag04}
% \end{equation}
% 
% \noindent Now, we use the definition of complex power where $\left( I_{mn}^{\phi} \right)^{*} = S_{mn}^{\phi} / V_{n}^{\phi}$, and define the term $\gamma_{n}^{\phi \psi} = V_{n}^{\phi} / V_{n}^{\psi}$, thus expand \eqref{eq:mag04} to \eqref{eq:mag05}:
% % , with $\gamma_{n}^{\phi \psi} = \gamma_{n}^{\psi \phi} = 0$ if $\phi \notin \mathcal{P}_{n}$ and thus we obtain:
% \begin{equation}
% \begin{aligned}
% 	& \left( \mathbf{Z}_{mn} \mathbf{I}_{mn} \right)^{*} \circ \mathbf{V}_{n} = \ldots
%     \\
%     & \qq
%     \begin{bmatrix}
%     	(Z_{mn}^{aa})^{*} S_{mn}^{a} + \gamma_{n}^{ab} (Z_{mn}^{ab})^{*} S_{mn}^{b} + \gamma_{n}^{ac} (Z_{mn}^{ac})^{*} S_{mn}^{c} \\
%         \gamma_{n}^{ba} (Z_{mn}^{ba})^{*} S_{mn}^{a} + (Z_{mn}^{bb})^{*} S_{mn}^{b} + \gamma_{n}^{bc} (Z_{mn}^{bc})^{*} S_{mn}^{c} \\
%         \gamma_{n}^{ca} (Z_{mn}^{ca})^{*} S_{mn}^{a} + \gamma_{n}^{cb} (Z_{mn}^{cb})^{*} S_{mn}^{b} + (Z_{mn}^{cc})^{*} S_{mn}^{c}
%     \end{bmatrix}
% \end{aligned}
% \label{eq:mag05}
% \end{equation}
% 
% \begin{equation}
% 	\mathbf{I}_{mn}^{*} = \mathbf{S}_{mn} \circ 1 / \mathbf{V}_{n}
% \end{equation}
% 
% PHASE POWER RX END
% \begin{equation}
% 	\left( I_{mn}^{\phi} \right)^{*} = S_{mn}^{n,\phi} / V_{n}^{\phi}
% \end{equation}
% 
% VOLTAGE RATIO
% \begin{equation}
% 	\gamma_{n}^{\phi \psi} = V_{n}^{\phi} / V_{n}^{\psi}
% \end{equation}
% 
% MAYBE SKIP THIS STEP?
% \begin{equation}
% \begin{aligned}
% 	& \mathbf{E}_{m} = \mathbf{E}_{n} + \mathbf{H}_{mn} + \ldots \\
%     & 2 \Re
%     \left\{
%     \begin{bmatrix}
%     	(Z_{mn}^{aa})^{*} S_{mn}^{a} / V_{n}^{a} + (Z_{mn}^{ab})^{*} S_{mn}^{b} / V_{n}^{b} + (Z_{mn}^{ac})^{*} S_{mn}^{c} / V_{n}^{c} \\
%         (Z_{mn}^{ba})^{*} S_{mn}^{a} / V_{n}^{a} + (Z_{mn}^{bb})^{*} S_{mn}^{b} / V_{n}^{b} + (Z_{mn}^{bc})^{*} S_{mn}^{c} / V_{n}^{c} \\
%         (Z_{mn}^{ca})^{*} S_{mn}^{a} / V_{n}^{a} + (Z_{mn}^{cb})^{*} S_{mn}^{b} / V_{n}^{b} + (Z_{mn}^{cc})^{*} S_{mn}^{c} / V_{n}^{c}
%     \end{bmatrix}
%     \circ
%     \begin{bmatrix}
%     	V_{n}^{a} \\ V_{n}^{b} \\ V_{n}^{c}
%     \end{bmatrix}
%     \right\}
% \end{aligned}
% \end{equation}
% 
% 
% KEEP THIS STEP, WHAT ABOUT S NODE n SUPER OR SUBSCRIPTS?
% \textcolor{red}{PICK ONE OF THESE EQUATIONS}
% \begin{equation}
% 	\mathbf{E}_{m} = \mathbf{E}_{n} + \mathbf{H}_{mn} +
%     2 \Re
%     \left\{
%     \sum_{\phi \in \{a,b,c\}}
%     \begin{bmatrix}
% %         \sum_{\phi in \{a,b,c\}}
%         V_n^{a} (Z_{mn}^{a \phi} )^{*} S_{mn}^{\phi} / V_n^{\phi} \\
% %         \sum_{\phi in \{a,b,c\}}
%         V_n^{b} (Z_{mn}^{b \phi} )^{*} S_{mn}^{\phi} / V_n^{\phi} \\
% %         \sum_{\phi in \{a,b,c\}}
%         V_n^{c} (Z_{mn}^{c \phi} )^{*} S_{mn}^{\phi} / V_n^{\phi}
%     \end{bmatrix}
%     \right\}
% \end{equation}
% 
% \begin{equation}
% 	\mathbf{E}_{m} = \mathbf{E}_{n} + \mathbf{H}_{mn} +
%     2 \Re
%     \left\{
%     \sum_{\phi \in \{a,b,c\}}
%     \begin{bmatrix}
% %         \sum_{\phi \in \{a,b,c\}}
%         \gamma_n^{a \phi} (Z_{mn}^{a \phi} )^{*} S_{mn}^{\phi} \\
% %         \sum_{\phi \in \{a,b,c\}}
%         \gamma_n^{b \phi} (Z_{mn}^{b \phi} )^{*} S_{mn}^{\phi} \\
% %         \sum_{\phi \in \{a,b,c\}}
%         \gamma_n^{c \phi} (Z_{mn}^{c \phi} )^{*} S_{mn}^{\phi}
%     \end{bmatrix}
%     \right\}
% \end{equation}
% 
% \begin{equation}
% \begin{aligned}
% 	& \mathbf{E}_{m} = \mathbf{E}_{n} + \mathbf{H}_{mn} + \ldots \\
%     & 2 \Re
%     \left\{
%     \begin{bmatrix}
%     	(Z_{mn}^{aa})^{*} S_{mn}^{a} + \gamma_{n}^{ab} (Z_{mn}^{ab})^{*} S_{mn}^{b} + \gamma_{n}^{ac} (Z_{mn}^{ac})^{*} S_{mn}^{c} \\
%         \gamma_{n}^{ba} (Z_{mn}^{ba})^{*} S_{mn}^{a} + (Z_{mn}^{bb})^{*} S_{mn}^{b} + \gamma_{n}^{bc} (Z_{mn}^{bc})^{*} S_{mn}^{c} \\
%         \gamma_{n}^{ca} (Z_{mn}^{ca})^{*} S_{mn}^{a} + \gamma_{n}^{cb} (Z_{mn}^{cb})^{*} S_{mn}^{b} + (Z_{mn}^{cc})^{*} S_{mn}^{c}
%     \end{bmatrix}
%     \right\}
% \end{aligned}
% \end{equation}
% 
% \noindent The $3 \times 1$ vector on the RHS can be separated into a $3 \times 3$ matrix multiplied by the $3 \times 1$ vector $\mathbf{S}_{mn}$.
% \begin{equation}
% \begin{aligned}
% 	& \mathbf{E}_{m} = \mathbf{E}_{n} + \mathbf{H}_{mn} + \ldots \\
%     & 2 \Re
%     \left\{
%     \begin{bmatrix}
%     	(Z_{mn}^{aa})^{*} & \gamma_{n}^{ab} (Z_{mn}^{ab})^{*} & \gamma_{n}^{ac} (Z_{mn}^{ac})^{*} \\
%         \gamma_{n}^{ba} (Z_{mn}^{ba})^{*} & (Z_{mn}^{bb})^{*} & \gamma_{n}^{bc} (Z_{mn}^{bc})^{*}\\
%         \gamma_{n}^{ca} (Z_{mn}^{ca})^{*} & \gamma_{n}^{cb} (Z_{mn}^{cb})^{*} & (Z_{mn}^{cc})^{*}
%     \end{bmatrix}
%     \begin{bmatrix}
%     	S_{mn}^{a} \\ S_{mn}^{b} \\ S_{mn}^{c}
%     \end{bmatrix}
%     \right\}
% \end{aligned}
% \end{equation}
% \begin{equation}
% \begin{aligned}
% 	& \left( \mathbf{Z}_{mn} \mathbf{I}_{mn} \right)^{*} \circ \mathbf{V}_{n} = \ldots
%     \\
%     & \quad
%     \begin{bmatrix}
%     	(Z_{mn}^{aa})^{*} & \gamma_{n}^{ab} (Z_{mn}^{ab})^{*} & \gamma_{n}^{ac} (Z_{mn}^{ac})^{*} \\
%         \gamma_{n}^{ba} (Z_{mn}^{ba})^{*} & (Z_{mn}^{bb})^{*} & \gamma_{n}^{bc} (Z_{mn}^{bc})^{*}\\
%         \gamma_{n}^{ca} (Z_{mn}^{ca})^{*} & \gamma_{n}^{cb} (Z_{mn}^{cb})^{*} & (Z_{mn}^{cc})^{*}
%     \end{bmatrix}
%     \begin{bmatrix}
%     	S_{mn}^{a} \\ S_{mn}^{b} \\ S_{mn}^{c}
%     \end{bmatrix}
% \end{aligned}
% \label{eq:mag06}
% \end{equation}
% we can use the definition of the HP to separate the $3 \times 3$ matrix into two $3 \times 3$ matrices as in:
% \begin{equation}
% 	\left( \mathbf{Z}_{mn} \mathbf{I}_{mn} \right)^{*} \circ \mathbf{V}_{n} = \left( \Gamma_{n} \circ \mathbf{Z}_{mn}^{*} \right) \mathbf{S}_{mn}
% 	\label{eq:mag07}
% \end{equation}
% 
% Placing \eqref{eq:mag07} back into \eqref{eq:mag03} gives:
% \begin{equation}
% \begin{aligned}
% 	\mathbf{Y}_{m} = \mathbf{Y}_{n} + 2 \Re \left\{ \left( \Gamma_{n} \circ \mathbf{Z}_{mn}^{*} \right) \mathbf{S}_{mn} \right\} + \mathbf{H}_{mn}
% \end{aligned}
% \label{eq:mag08}
% \end{equation}
% 
% \noindent Finally, we apply the real part operator $\Re(\cdot)$ on the RHS, separating the complex power vector into its active and reactive components, $\mathbf{S}_{mn} = \mathbf{P}_{mn} + j \mathbf{Q}_{mn}$, to arrive at:
\begin{equation}
\begin{gathered}
	\mathbf{y}_{m} = \mathbf{y}_{n} + 2 \mathbf{M}_{mn} \mathbf{P}_{mn} - 2 \mathbf{N}_{mn} \mathbf{Q}_{mn} + \mathbf{H}_{mn} \\
    \mathbf{M}_{mn} = \Re \left\{ \Gamma_{n} \circ \mathbf{Z}_{mn}^{*} \right\},
    \mathbf{N}_{mn} = \Im \left\{ \Gamma_{n} \circ \mathbf{Z}_{mn}^{*} \right\} \,,
\end{gathered}
\label{eq:mag09}
\end{equation}
where $\Gamma_{n} = \mathbf{V}_{n} \left( 1 / \mathbf{V}_{n} \right)^{T} \in \mathbb{C}^{3 \times 3}$ represents a matrix with voltage balance ratios across all phases at node $n$. Hence, we have that $\Gamma_{n}\left( \phi, \phi \right) = 1$ and  $\Gamma_{n}\left( \phi, \psi \right) = V_n^{\phi}/V_n^{\psi} \triangleq \gamma_{n}^{\phi \psi}$. Furthermore, $\mathbf{H}_{mn} = \left( \mathbf{Z}_{mn} \mathbf{I}_{mn} \right) \circ \left( \mathbf{Z}_{mn} \mathbf{I}_{mn} \right)^{*} = \left( \mathbf{V}_{m} - \mathbf{V}_{n} \right) \circ \left( \mathbf{V}_{m} - \mathbf{V}_{n} \right)^{*}$ is a $3 \times 1$ real-valued vector representing higher-order terms. 
Notice that we have separated the complex power vector into its active and reactive components, $\mathbf{S}_{mn} = \mathbf{P}_{mn} + j \mathbf{Q}_{mn}$.

This nonlinear and nonconvex system is difficult to incorporate into a state estimation or optimization formulation without the use of convex relaxations. Following the analysis in \cite{gan_convex_2014}, we apply two approximations. The first approximation is legitimized by the fact that the high order term $\mathbf{H}_{mn}$ is negligible, such that $\mathbf{H}_{mn} = \left[ 0 , \ 0 , \ 0 \right]^{T}$. The second approximation assumes that node voltages are ``nearly balanced" such that:
% \begin{equation}
% 	\begin{array}{lr}
%     	\gamma_{n}^{ab} = \alpha \quad \gamma_{n}^{bc} = \alpha \quad \gamma_{n}^{ac} = \alpha^{2} \\
%         \gamma_{n}^{ba} = \alpha^{2} \quad \gamma_{n}^{cb} = \alpha^{2} \quad \gamma_{n}^{ca} = \alpha
%     \end{array}
% 	\forall n \in \mathcal{N} \, ,
%     \label{eq:gammaalpha}
% \end{equation}
% 
% \noindent where $\alpha = 1 \angle 120 \degree = \frac{1}{2} ( -1 + j \sqrt{3} )$ and $\alpha^{-1} = \alpha^{2} = \alpha^{*} = 1 \angle 240 \degree$. Hence, we can also write
\begin{equation}
	\Gamma
    =
    \begin{bmatrix}
    	1 & \gamma_{n}^{ab} & \gamma_{n}^{ab} \\
        \gamma_{n}^{ba} & 1 & \gamma_{n}^{bc} \\
        \gamma_{n}^{ca} & \gamma_{n}^{cb} & 1
    \end{bmatrix}
    =
    \begin{bmatrix}
    	1 & \alpha & \alpha^{2} \\
        \alpha^{2} & 1 & \alpha \\
        \alpha & \alpha^{2} & 1
    \end{bmatrix}
	\forall n \in \mathcal{N} \,,
    \label{eq:gammaalpha}
\end{equation}
\noindent where $\alpha = 1 \angle 120 \degree = \frac{1}{2} ( -1 + j \sqrt{3} )$ and $\alpha^{-1} = \alpha^{2} = \alpha^{*} = 1 \angle 240 \degree = \frac{1}{2} ( -1 - j \sqrt{3} )$.
Applying the approximations for $\mathbf{H}_{mn}$ and $\Gamma_{n}$ to \eqref{eq:mag09}, we arrive at a linear system of equations:
\begin{equation}
	\mathbf{y}_{m} \approx \mathbf{y}_{n} + 2 \mathbf{M}_{mn} \mathbf{P}_{mn} - 2 \mathbf{N}_{mn} \mathbf{Q}_{mn} \,, \text{ with}
    \label{eq:mag10}
\end{equation}
\begin{equation}
\begin{aligned}
	2 & \mathbf{M}_{mn}
    = \ldots \\
	& \begin{bmatrix}
		2 r_{mn}^{aa} & -r_{mn}^{ab} + \sqrt{3} x_{mn}^{ab} & -r_{mn}^{ac} - \sqrt{3} x_{mn}^{ac} \\
		-r_{mn}^{ba} - \sqrt{3} x_{mn}^{ba} & 2 r_{mn}^{bb} & -r_{mn}^{bc} + \sqrt{3} x_{mn}^{bc} \\
		-r_{mn}^{ca} + \sqrt{3} x_{mn}^{ca} & -r_{mn}^{cb} - \sqrt{3} x_{mn}^{cb} & 2 r_{mn}^{cc}
	\end{bmatrix} \,,
\end{aligned}
\label{eq:Mmn}
\end{equation}
% \begin{equation}
% \begin{aligned}
% 	2 & \mathbf{M}_{mn}
%     = \ldots \\
% 	& - \begin{bmatrix}
% 		-2 r_{mn}^{aa} & r_{mn}^{ab} - \sqrt{3} x_{mn}^{ab} & r_{mn}^{ac} + \sqrt{3} x_{mn}^{ac} \\
% 		r_{mn}^{ba} + \sqrt{3} x_{mn}^{ba} & - 2 r_{mn}^{bb} & r_{mn}^{bc} - \sqrt{3} x_{mn}^{bc} \\
% 		r_{mn}^{ca} - \sqrt{3} x_{mn}^{ca} & r_{mn}^{cb} + \sqrt{3} x_{mn}^{cb} & - 2 r_{mn}^{cc}
% 	\end{bmatrix}
% \end{aligned}
% \label{eq:Mmn}
% \end{equation}
\begin{equation}
\begin{aligned}
	2 & \mathbf{N}_{mn}
    = \ldots \\
	& \begin{bmatrix}
		-2 x_{mn}^{aa} & x_{mn}^{ab} + \sqrt{3} r_{mn}^{ab} & x_{mn}^{ac} - \sqrt{3} r_{mn}^{ac} \\
		x_{mn}^{ba} -\sqrt{3} r_{mn}^{ba} & -2 x_{mn}^{bb} & x_{bc} + \sqrt{3} r_{mn}^{bc}\\
		x_{mn}^{ca} + \sqrt{3} r_{mn}^{ca} & x_{mn}^{cb} -\sqrt{3} r_{mn}^{cb} & -2 x_{mn}^{cc}
	\end{bmatrix} \,.
\end{aligned}
\label{eq:Nmn}
\end{equation}

% The derivation we have presented is for a line with three phases. For a line with one or two phases, \eqref{eq:mag10} - \eqref{eq:Nmn} should be indexed by $\mathcal{P}_{mn}$, 
% where the vectors $\mathbf{E}_{m}$, $\mathbf{E}_{n}$, $\mathbf{P}_{mn}$, and $\mathbf{Q}_{mn}$ are indexed as $\left[ \cdot \right]_{\mathcal{P}_{mn}}$ and matrices $\mathbf{M}_{mn}$ and $\mathbf{N}_{mn}$ are indexed as $\left[ \cdot \right]_{\mathcal{P}_{mn},\mathcal{P}_{mn}}$.
% where rows of \eqref{eq:mag10} - \eqref{eq:Nmn}, and columns of $\mathbf{M}_{mn}$ and $\mathbf{N}_{mn}$, corresponding to $\phi \notin \mathcal{P}_{mn}$ are removed.

We present the full set of equations that comprise a linearized model for unbalanced power flow. 
We named these the \emph{LinDist3Flow} equations, as developed in~\cite{arnold_optimal_2016,sankur_linearized_2016,sankur_optimal_2018}.

\begin{tcolorbox}[ams gather]
\textbf{LinDist3Flow Equations for Three-Phase Networks} \nonumber \\
\text{Per phase node complex load:} \nonumber
\\
s_{n}^{\phi} \left( y_{n}^{\phi} \right) = \left( \beta_{S,n}^{\phi} + \beta_{Z,n}^{\phi} y_{n}^{\phi} \right) d_{n}^{\phi} + u_{n}^{\phi} - j c_{n}^{\phi} \,, \label{eqn:nodallin} \\
\forall \phi \in \mathcal{P}_{n}, \, \forall n \in \mathcal{N} 
\nonumber
\\
% \mathbf{s}_{n} \left( \mathbf{V}_{n} \right) = \left( \mathbf{B}_{S,n} + \mathbf{B}_{Z,n} \circ \mathbf{E}_{n} \right) \circ \mathbf{d}_{n} + \mathbf{w}_{n} - j \mathbf{c}_{n}
% \label{eqn:sVlin02}
% \\
\text{Branch power flow:} \nonumber
\\
\sum_{l:(l,m) \in \mathcal{E}} \mathbf{S}_{lm} \approx \mathbf{s}_{m} + \sum_{n:(m,n) \in \mathcal{E}} \mathbf{S}_{mn} \,, \forall m \in \mathcal{N}
\label{eqn:powerlin}
\\
\text{Magnitude and angle equations:} \nonumber
\\
\left[ \mathbf{y}_{m} \approx \mathbf{y}_{n} + 2 \mathbf{M}_{mn} \mathbf{P}_{mn} - 2 \mathbf{N}_{mn} \mathbf{Q}_{mn} \right]_{\mathcal{P}_{mn}} \,, 
\label{eqn:maglin}
\\
\left[ \Theta_{m} \approx \Theta_{n} - \mathbf{N}_{mn} \mathbf{P}_{mn} - \mathbf{M}_{mn} \mathbf{Q}_{mn} \right]_{\mathcal{P}_{mn}} \,,
\label{eqn:anglelin}
\\
\text{with }\left[ \mathbf{M}_{mn}= \Re \left\{ \Gamma \mathbf{Z}_{mn}^{*} \right\} , \
\mathbf{N}_{mn}= \Im \left\{ \Gamma \mathbf{Z}_{mn}^{*} \right\} \right]_{\mathcal{P}_{mn}} \nonumber \\
\forall (m,n) \in \mathcal{E} \,. \label{eqn:MmnNmnlin}
\end{tcolorbox}

Here, we have embraced a load model with a fixed voltage sensitivity (as parameterized with $\beta_{S,n}^{\phi}, \beta_{Z,n}^{\phi}$), with $d_{n}^{\phi}$ denoting demand, $u_{n}^{\phi} := u_n^{p,\phi} + j u_n^{q,\phi}$ the controllable power injection and $c_{n}^{\phi}$ a possible capacitor bank.

The accuracy of the approximations in the power and voltage magnitude equations has been investigated in \cite{gan_convex_2014} and \cite{robbins_optimal_2016-1}. In~\cite{sankur_optimal_2018}, we perform a Monte Carlo analysis to explore the level of error introduced by the voltage angle equation assumptions.

\section{Three-phase Optimal Power Flow}

\subsection*{Voltage Balancing}
\label{sec:sim_voltage_balance}

Although the \textit{LinDist3Flow} equations allow for a flexible OPF framework comparable to the one presented for single-phase networks above, here we focus on one instance to demonstrate the generalization of decentralized OPF to three-phase unbalanced systems.
We remodel an instance first presented in~\cite{sankur_linearized_2016} that demonstrated OPF for balancing voltage magnitudes on an unbalanced radial distribution feeder.  
This is an important objective as many three phase loads (induction motors for instance) are sensitive to high levels of voltage imbalance. 
Furthermore, 3-phase voltage regulation equipment may actuate based on single phase measurements, and significant imbalances can lead to improper operation of these devices. 
% This simulation incorporated both constant power and constant impedance loads as defined in \cite{_ieee_2017} for the 13 node case.  
The problem is defined as
\begin{equation}
\begin{array}{rl}
% \begin{aligned}
  \underset{y_{n}^{\phi},P_{mn}^{\phi},Q_{mn}^{\phi},u_{n}^{\phi}} {\text{min}}
  % & & P_{0}\\
%   & & \sum_{n \in H} \left[ \sum_{ \substack{ {\phi, \psi} \\ {\phi \neq \psi} }} ( y_{n}^{\phi} - y_{n}^{\psi} )^{2} + \rho \sum_{\phi} \left| w_{n}^{\phi} \right|^{2} \right]  \\
  & \sum_{n \in \N} \left[ \sum_{\phi \neq \psi} ( y_{n}^{\phi} - y_{n}^{\psi} )^{2} + \rho \sum_{\phi} \left| u_{n}^{\phi} \right|^{2} \right] \nonumber \\
  \text{s.t.}
  & \eqref{eqn:nodallin} \,, \eqref{eqn:powerlin} \,, \eqref{eqn:maglin} \,, \underline{y} \le y_{n}^{\phi} \le \overline{y}, \nonumber \\
  &  \left| u_{n}^{\phi} \right| \le \overline{u}, \quad \forall n \in \N \,,
% \end{aligned}
\label{eq:OP3F}
\end{array}
\end{equation}

\noindent where $\phi,\psi \in \{ a,b,c\}$. 
The parameter $\rho$ is a penalty on control action set to $0.01$. 
\cite{sankur_linearized_2016}~showed the effectiveness of the \textit{LinDist3Flow} model in drastically reducing voltage imbalance across phases, and we will aim to reproduce these results in Section~\ref{sec:results_3ph}. 

% to investigate the benefit of the iterative algorithm of Section \ref{subsec:analysis_iter}, as listed below:
% \begin{itemize}
% 	\item[-] Case 0 - The uncontrolled, or base case (see Fig. \ref{fig:s2bc}).
% 	\item[-] Case 1 - OPF initialized as per assumptions outlined in Section \ref{subsec:analysis_nominal} with $\gamma_{n}^{\phi \psi} = \sigma \text{ or } \sigma^{2}$, and $\mathbb{L}_{mn} = \mathbb{H}_{mn}  = 0_{3 \times 1}$. See Fig. \ref{fig:s2c1}
%     \item[-] Case 2 - OPF solved as outlined in Section \ref{subsec:analysis_iter}.  See Fig. \ref{fig:s2c3}
% \end{itemize}

% \setlength{\abovedisplayskip}{0pt}
% \setlength{\belowdisplayskip}{0pt}

% It should be noted that comparison of either case to an SDP formulation of \eqref{eq:OPF2} was not possible as it is not, to the authors knowledge, possible to formulate a semidefinite program with this objective function.

% It can clearly be seen that for both Case 1 and Case 2, the voltage imbalance is drastically reduced compared to Case 0. In Case 1, the gap between phases a and b is reduced, however the magnitude of phase c remains lower throughout the feeder. In Case 2, the three phases are much more closely matched. We define voltage imbalance for the network as:
% \begin{equation}
% 	J (\mathbb{Y}) = 
% % 	\sum_{n \in H} \sum_{ \substack{ {\phi, \psi} \\ {\phi \neq \psi} }} ( y_{n}^{\phi} - y_{n}^{\psi} )^{2}
%     \sum_{n \in H} \sum_{\phi \neq \psi} ( y_{n}^{\phi} - y_{n}^{\psi} )^{2}
%     \label{eq:JV}
% \end{equation}

% % \setlength{\abovedisplayskip}{5pt}
% % \setlength{\belowdisplayskip}{-50pt}
% \setlength{\belowcaptionskip}{0pt}
% \setlength{\textfloatsep}{5pt}
% \begin{figure}[ht!]
% 	\centering
% 	\includegraphics[width=0.49\textwidth]{s2bc.eps}
% 	\caption{Voltage profile of IEEE 13 node feeder with zero control.}
% 	\label{fig:s2bc}
%     \begin{subfigure}[b]{0.49\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{s1sdp.eps}
%         \caption{Voltage profile of IEEE 13 node feeder with SDP control.}
%         \label{fig:s1sdp}
%     \end{subfigure}
%     \\
%     \begin{subfigure}[b]{0.49\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{s1lin.eps}
%         \caption{Voltage profile of IEEE 13 node feeder with control from \eqref{eq:OPF1}}
%         \label{fig:s1lin}
%     \end{subfigure}
%     \caption{Comparison of voltage profiles for feeder head real power minimization scenario.}
%     \label{fig:s1}
%     \begin{subfigure}[b]{0.49\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{s2c1.eps}
%         \caption{Voltage profile of IEEE 13 node feeder with \eqref{eq:OPF2} Case 1 control.}
%         \label{fig:s2c1}
%     \end{subfigure}
%     \\
%     \begin{subfigure}[b]{0.49\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{s2c3.eps}
%         \caption{Voltage profile of IEEE 13 node feeder with \eqref{eq:OPF2} Case 2 control.}
%         \label{fig:s2c3}
%     \end{subfigure}
%     \caption{Comparison of voltage profiles for voltage balancing scenario.}
%     \label{fig:s2}
% \end{figure}

% \noindent where $\phi,\psi \in  \{ a,b,c\}$ and $\mathbb{Y}$ is the set of all $\mathbb{Y}_{n}, \text{ } n \in H$. The voltage imbalance for Case 0 is 0.05443. The imbalance for Case 1 is 8.334e-4, and the imbalance for Case 2 is 8.054e-4, a 3.36 \% improvement over Case 1.



%% From TSG journal paper
% In addition to single-phase experiments, we will also consider some experiments on three-phase unbalanced networks.
% We adapt the OPF formulation from~\cite{sankur_optimal_2018}.
% In this paper, the objective was to close a switch in order to connect two networks on line. 
% To minimize large instantaneous power transfers across the switch upon closing, one needs to match the voltage phasors at the ends of the open switch. 
% To this end, \cite{sankur_optimal_2018} proposed the following OPF to minimize the voltage phasor difference between one or more nodes and the respective reference at each node, while providing feeder voltage support:
% \begin{align}
% \begin{aligned}
% & \underset{\substack{u_{n}^{\phi}, v_{n}^{\phi}, E_{n}^{\phi} \\ \theta_{n}^{\phi}, P_{n}^{\phi}, Q_{n}^{\phi}}} {\text{minimize}}
% & & \rho_{E} C_{E} + \rho_{\theta} C_{\theta} + \rho_{w} C_{w} \\
% & \text{subject to}
% & & \eqref{eqn:sVlin01}, \eqref{eqn:powerlin}, \eqref{eqn:maglin}, \eqref{eqn:anglelin}, \eqref{eqn:MmnNmnlin} \\
% & & & \underline{E} \le E_{n}^{\phi} \le \overline{E} \,, \ \forall \phi \in \mathcal{P}_{n}, \, \forall n \in \mathcal{N} \\
% & & & \mathbf{E}_{\infty} = \left[ 1, \ 1, \ 1 \right]^{T} \\
% % & & & \Theta_{\infty} = \left[ 0^{\circ}, \ 240^{\circ}, \ 120^{\circ} \right]^{T} \\
% & & & \Theta_{\infty} = \left[ 0, \ -2\pi/3, \ 2\pi/3 \right]^{T} \\
% & & & \left| w_{n}^{\phi} \right| \le \overline{w}_{n}^{\phi} \,, \ \forall \phi \in \mathcal{P}_{n}, \, \forall n \in \mathcal{G}
% \, ,
% \end{aligned}
% \label{eqn:OPF1}
% \end{align}
% % \noindent where
% \begin{align}
% C_{E} &= \sum_{\phi \in \mathcal{P}_{1680,2680}} {\left( E_{1680}^{\phi} - E_{2680}^{\phi} \right)}^{2}
% \, , \label{eqn:OPFCE} \\
% C_{\theta} &= \sum_{\phi \in \mathcal{P}_{1680,2680}} {\left( \theta_{1680}^{\phi} - \theta_{2680}^{\phi} \right)}^{2}
% \, , \label{eqn:OPFCtheta} \\
% C_{w} &= \sum_{n \in \mathcal{G}} \sum_{\phi \in \mathcal{P}_{n}} {\left| w_{n}^{\phi} \right|}^{2}
% \, \,. \label{eqn:OPFCw}
% \end{align}
% The OPF objective function is a weighted sum of three terms: $C_{E}$ is the sum of squared voltage magnitude differences squared, $C_{\theta}$ is the sum of voltage angle differences squared, and $C_{w}$ is the sum of the squared magnitudes of all DER dispatch, to avoid applying excessive amounts of control. 
% Constraints of lower and upper voltage magnitude bounds were imposed as $0.95 \le \left| V_{n}^{\phi} \right| \le 1.05 \ \forall \phi \in \mathcal{P}_{n}, \forall n \in \mathcal{N}$ such that $\underline{E} = 0.9025$ and $\overline{E} = 1.1025$. 
% Additionally, DER dispatch is constrained by its apparent power capacity, $\overline{w}_{n}^{\phi}$.


\section{Results for Three-Phase Optimal Power Flow}
\label{sec:results_3ph}
We also show the efficacy of Decentralized OPF for three-phase unbalanced networks, by learning and reconstructing the solutions~$u_{n}^{p,\phi},u_{n}^{q,\phi}$, with $\phi \in \{ a,b,c\}$, of the centralized OPF problem~\eqref{eq:OP3F}, as formulated in Section~2 of the main paper.
The feeder model used here is the IEEE 13 node test feeder~\cite{_ieee_2017}.
Figure~\ref{fig:Result3Phase} shows the results of applying Decentralized OPF to balance voltage magnitudes across phases for a scenario with a significant gap between phase~$b$ and phase~$c$ of $\approx 0.1$p.u..
We see that the voltage magnitudes are tightly balanced across the network. Notice that in order to balance the large gap in the lower half of the feeder (nodes 671, 692, 675, 680, 684), a small increase in gap is incurred in the left upper radial (nodes 645, 646).
Similar to the results for single-phase networks, the Decentralized OPF method also performs well at locally reconstructing OPF solutions in three-phase unbalanced networks, further validating its promise to serve as a new paradigm for regulating voltage and power flow in distribution networks.

\begin{figure}[h!]
\centering
\includegraphics[trim=0.5cm 0 1.5cm 0,width=.48\textwidth]{rbic_figs/20180325_Voltage_Balancing.eps}
%\includegraphics[width=.5\textwidth]{rbic_figs/VoltBandwidths.eps}
\caption{Voltage magnitude balancing. In grey, voltage magnitudes across three phases without control. In black, voltage magnitudes across three phases applying decentralized OPF.}
\label{fig:Result3Phase}
\end{figure}



